Question-type Driven Question Generation

Question generation is a challenging task which aims to ask a question based on an answer and relevant context. The existing works suffer from the mismatching between question type and answer, i.e. generating a question with type $how$ while the answer is a personal name. We propose to automatically predict the question type based on the input answer and context. Then, the question type is fused into a seq2seq model to guide the question generation, so as to deal with the mismatching problem. We achieve significant improvement on the accuracy of question type prediction and finally obtain state-of-the-art results for question generation on both SQuAD and MARCO datasets.

==> temp.tex <==
        \midrule
        \textbf{Context:} concentrated o 2 will allow combustion to proceed rapidly and energetically . \\
        \textbf{Answer:} combustion \\
        \textbf{Reference:} what will concentrated oxygen greatly speed up ? \\
        \textbf{Baseline:} concentrated o 2 will allow what to proceed rapidly and energetically ? \\
        \textbf{Joint-model:} what does concentrated o 2 will allow to proceed rapidly and energetically ? \\
        
, which is caculated as follow:
\begin{empheq}{align}
\small\text{BQWA} &= \small\frac{\text{\#(right question words prediction)}}{\text{\#(question words as beginning)}}
\end{empheq}

\section{Related Work}

Previous work of QG was mainly tackled by two approaches: rule-based method and neural network model. Rule-based method can simply resort to two categories, template-based slot filling and syntactic transformation, e.g. \cite{heilman2010good,chali2015towards,labutov2015deep}. They rely on handcrafted rules that are expensive to create and lack of generalization ability, meanwhile these approaches cannot apprehend the diversity meaning of human generated questions.

Recently, \cite{du2017learning} pioneered the work of automatic QG on SQuAD using a seq2seq model with attention mechanism, this work outperformed the previous state-of-the-art rule-based system. \cite{Zhou2017Neural} utilized rich features and incorporated copy mechanism. Based on this work, \cite{sun2018answer-focused} proposed an answer-focused model to generate proper question words combined with a position-aware model to put more emphasis on answer surrounded context. \cite{song2018leveraging} introduced multi-perspective matching strategies into the seq2seq model to capture rich potential correlations between the text and target answer. \cite{zhao2018paragraph-level} aggregated paragraph-level information with gated self-attention mechanism to help sentence-level QG. Another line of work is to deal with question answering and question generation together \cite{tang2017question,duan2017question}.

Besides the above work that focus on answer-aware question generation， \cite{subramanian2018neural} (another citation??) tried to generate questions from text without answer as input, where the model first learns to predict the important key phrases or sentences worthy to be questioned and then generate questions. Their pipeline approaches are different from our joint model, since our neural network aims to obtain a powerful sentence representation     

\cite{Caruana:1998:ML:296635.296645} described the idea of \textbf{MTL} (multi-task learning) which is effective for improving generalization performance via related task by introducing more data and semantic information to the neural network. Several recent works in NLP have adopted multi-task learning, e.g. \cite{rei2017semi-supervised,guo2018soft,ye2018semi-supervised,liu2018neural,chen2018joint}, and MTL was proved to be fruitful for many NLP tasks, both on extractive and abstractive tasks.

However, nobody attempts to incorporate MTL in question generation. Despite so many inspiring works have been done on this task, their specified designed model helpful to solve particular drawback of previous work based on the observation of generated results of particular dataset cannot the generalization ability, it may fail to work as design if the dataset change. To solve this problem, we introduce two auxiliary tasks for MTL to generate informative questions.



